Guided Incremental Local Densification for Accelerated Sampling-based Motion Planning

Sampling-based motion planners rely on incremental densification to discover progressively shorter paths. After computing feasible path $\xi$ between start $x_s$ and goal $x_t$, the Informed Set (IS) prunes the configuration space $\mathcal{C}$ by conservatively eliminating points that cannot yield shorter paths. Densification via sampling from this Informed Set retains asymptotic optimality of sampling from the entire configuration space. For path length $c(\xi)$ and Euclidean heuristic $h$, $IS = \{ x | x \in \mathcal{C}, h(x_s, x) + h(x, x_t) \leq c(\xi) \}$. Relying on the heuristic can render the IS especially conservative in high dimensions or complex environments. Furthermore, the IS only shrinks when shorter paths are discovered. Thus, the computational effort from each iteration of densification and planning is wasted if it fails to yield a shorter path, despite improving the cost-to-come for vertices in the search tree. Our key insight is that even in such a failure, shorter paths to vertices in the search tree (rather than just the goal) can immediately improve the planner's sampling strategy. Guided Incremental Local Densification (GuILD) leverages this information to sample from Local Subsets of the IS. We show that GuILD significantly outperforms uniform sampling of the Informed Set in simulated $\mathbb{R}^2$, $SE(2)$ environments and manipulation tasks in $\mathbb{R}^7$.

==> algorithms/alg_banditbeaconselector.tex <==
% !TEX root = ../root.tex
%------------------------------------------%
% Algorithm E3: BanditBeaconSelector
%------------------------------------------%
\begin{algorithm}[t]
\SetAlgoLined
\setstretch{1.2}
\caption{\texttt{BanditBeaconSelector}}
\label{alg:bandit}
\SetKwInOut{Input}{Input}
% \vspace{1mm}
\SetKwInOut{Parameter}{Parameter}
\SetKwInOut{Output}{Output}
\Input{$K, \mathcal{B}_t, \mathbf{c}(t), \gamma$}
\Output{Beacon $i$}

Initialize beacons to uniform: $ \forall i \in \mathcal{B}$ $\alpha_i=1, \beta_i=1$ \\

Initialize beacons $s$ and $t$ with $\beta=10$ \\

\For{$t = 1:T$}
{
    $\sigma = \emptyset $ \\
    \For{$i = 1:K$}
    {
        $p_i(t) \sim \texttt{Beta}(\alpha_i, \beta_i)$ \\
        $\sigma \xleftarrow{+} p_i(t)$ \\
    }
    
    Rank $\sigma$ in descending order \\
    Select beacon:  $i = \argmax{(\sigma \cap \mathcal{B}_t)}$ \\
    Observe shortest path cost $c_i(t)$ \\
    \If{$c_i(t) < c_{i-1}(t)$}
    {
        $\alpha_i \gets \alpha_i + \gamma$
    }
    \Else
    {
        $\beta_i \gets \beta_i + \gamma$ %this must change
        % add description of gamma and At
        % should we shift reward to cost?
    }
    
}
\end{algorithm}

==> algorithms/alg_exp3.tex <==
% !TEX root = ../root.tex
%------------------------------------------%
% Algorithm E?: Exp3
%------------------------------------------%
\begin{algorithm}[t]
\SetAlgoLined
\setstretch{1.2}
\caption{\texttt{Exp3}}
\label{alg:sample}
\SetKwInOut{Input}{Input}
% \vspace{1mm}
\SetKwInOut{Parameter}{Parameter}
\SetKwInOut{Output}{Output}
\Input{$K,\bold{x}(t),\gamma$}
\Output{Action $i,x_i(t),\hat{x}_{i_t}(t), w(t)$}
\For{$t = 1:T$}
{
    \For{$i = 1:K$}
    {
        $p_i(t) = (1-\gamma)\frac{w_i(t)}{\sum_{j=1}^K w_j(t)} + \frac{\gamma}{K}$
    }
    
    Draw next action $i_t$ randomly according to $p_i(t)$ \\
    Observe reward $x_i(t)$ \\
    $\hat{x}_{i_t}(t) \gets \frac{x_{i_t}(t)}{p_{i_t}(t)}$ \\
    $w_{i_t}(t+1) \gets w_{i_t}(t) e^{\gamma\hat{x}_{i_t}(t)/K}$ \\
    
    \For{$j = 1:K$ where $j \neq i$}
    {
         $w_{j_t}(t+1) \gets w_{j_t}(t)$
    }
}
\end{algorithm}

==> inputs/bandits.tex <==
% !TEX root = ../root.tex
\subsection{Bandit Beacon Selector}

%The characteristics of the beacon selection problem lead us to a bandit setting with two key assumptions: 1.) The action availability is stochastic. 2.) The payoff function of any particular action for any round is stochastic (and possibly adversarial). This is sometimes referred to as the `sleeping bandit' setting.

We assume a set of $\mathcal{B}$ beacons indexed by the integers $1, ..., K$. The goal of the algorithm \texttt{BanditBeaconSelector} is to select one bandit to be the beacon per round where each round $t$ is an iteration of the outer loop of \texttt{GuILD}. The output of \texttt{GuILD} specifies which of the beacons $\mathcal{B}^t \subseteq \mathcal{B} $ are available to be chosen for round $t$ as well as the cost of the shortest path $c_i(t)$ when beacon $i$ is selected.

Given only the available beacon candidates, $\mathcal{B}^t$, \texttt{BanditBeaconSelector} chooses a beacon $i \in \mathcal{B}^t $ and receives a cost $c_i$. Note that the bandit algorithm only receives the cost for the path induced by the single chosen beacon at round $t$.

\begin{comment}
The \texttt{BanditBeaconSelector} follows a strategy that compares the current performance to the best action list in hindsight. This is equivalent to minimizing regret with respect to the best action list $\sigma$. The particular notion of regret we use is the following:


\begin{equation} 
 \mathfrak{R} =
 \max\limits_{\sigma \in S_\mathcal{B}} \mathbb{E}_{\mathcal{B}^t}
 \left[ 
     \sum_{t=1}^{T}r^t [\sigma(\mathcal{B}^t)] 
 \right]
 - \sum_{t=1}^{T}r^t [\grave{b}^t] 
\end{equation} 

where $S_\mathcal{B}$ is the set of all permutations on $\mathcal{B}$ and $\grave{b}^t$ is the action taken by the algorithm at round $t$.
\end{comment}

We model the probability of any beacon being informative using a set of Beta distributions, maintaining a parameter set over all bandit $\theta_\mathcal{B} = (\alpha, \beta)_\mathcal{B}$. 
We construct priors for these distributions to encourage exploration of all bandits equally with the exception of the bandits corresponding to the start and goal vertex beacons. 
Over rounds $T$, each time a selected beacon results in a set from which the samples improve the shortest path cost $c(t)$, 
the algorithm increments the $\alpha$ parameter for this beacon's corresponding beta distribution by $\gamma$. 
Otherwise, the algorithm increments the corresponding $\beta$ parameter. 
This discourages the algorithm from picking beacons which consistently do not yield improvement in the shortest path cost. 
When selecting a bandit, the algorithm samples from all bandit beta distributions and 
ranks the bandits by probability of being informative. 
The highest ranking bandit contained within the current \texttt{InformedSet} is selected. 
As the number of rounds increases, 
the algorithm becomes amenable to selecting the start and goal vertex beacons. 
This behavior is desirable as we are confident that the \texttt{LocalSubsets} 
induced by using the start or goal as beacons will yield samples along the path, 
but we hope to explore and find even more attractive options early in the process. 
% Algorithm \ref{alg:bandit} shows the bandit beacon selection procedure. 
% \input{algorithms/alg_banditbeaconselector}


==> inputs/notes.tex <==
% !TEX root = ../root.tex
\section{Notes}
\begin{itemize}
\item Emphasis needs to be on path planning and reducing path length.
\item Should we say "although search algorithm can efficently compute optimal paths on graph, we require the sampling to provide the algorithm with a good graph?"
\item How do we define the connection radius correctly if we are not sampling from the informed set at all?
\end{itemize}


